LHC HXSWG interim recommendations to explore the coupling structure of a Higgs-like particle

This document presents an interim framework in which the coupling structure of a Higgs-like particle can be studied. After discussing different options and approximations, recommendations on specific benchmark parametrizations to be used to fit the data are given.

==> conclusions/conclusions.tex <==
\section{Conclusions}

